Fault Tolerant Control for Networked Mobile Robots

Teams of networked autonomous agents have been used in a number of applications, such as mobile sensor networks and intelligent transportation systems. However, in such systems, the effect of faults and errors in one or more of the sub-systems can easily spread throughout the network, quickly degrading the performance of the entire system. In consensus-driven dynamics, the effects of faults are particularly relevant because of the presence of unconstrained rigid modes in the transfer function of the system. Here, we propose a two-stage technique for the identification and accommodation of a biased-measurements agent, in a network of mobile robots with time invariant interaction topology. We assume these interactions to only take place in the form of relative position measurements. A fault identification filter deployed on a single observer agent is used to estimate a single fault occurring anywhere in the network. Once the fault is detected, an optimal leader-based accommodation strategy is initiated. Results are presented by means of numerical simulations and robot experiments.

==> sources/formationControl.tex <==
\section{Fault Identification and Accommodation Under Formation Control Dynamics}
\label{sec:formation}
\subsection{Formation Control Protocol}
In this section we expand the results from the previous two sections, assuming the robots performing a formation control task. We define a feasible set of distances between agents to be reached starting from the initial position and maintained over time. Let $\tilde{x}_i$ be the position of agent $i$ at equilibrium in a system attached to an arbitrary robot, the desired formation can be encoded by a matrix $\hat{H}\in\mathbb{R}^{n\times 2}$:
\begin{equation*}
\hat{H} = [\tau_1^T, \dots, \tau_n^T]^T
\end{equation*}
where:
\begin{equation*}
\tau_i = \sum_{j\in\mathcal{N}_i} \tilde{x}_i - \tilde{x}_j
\end{equation*}
is the sum of the relative distances between agent $i$ and its neighbor set. The final consensus-based formation control protocol subject to a faulty agent can then be written as:
\begin{eqnarray} \label{eq:formationFault}
\dot{x} &=& -L\,x + \hat{H} + \hat{F}_k \, \delta \, \nu, \qquad
\nu =
\begin{cases}
1 \,\, &\text{if} \,\, t \geq t_d \\
0 \,\, &\text{if} \,\, t <    t_d \\
\end{cases}
\end{eqnarray}

\subsection{Fault Identification Filter Revisited in Formation Control}
By performing the same transformation described in the Section~\ref{sec:fif}, we write the discrete model for the system as:
\begin{eqnarray}\label{eq:formationDiscrete}
\begin{aligned}
x_{k+1} &= (I -\Delta t \,L)\,x_k +\Delta t \, \hat{H}+ \Delta t \, \hat{F}_k \, \delta \\
&= A\,x_k + H + F_k \, \delta \\
y_k &= C_o\,x_k
\end{aligned}
\end{eqnarray}


\subsection{Fault Accommodation in Formation Control}
The solution of the minimization problem described in~\ref{sec:optimalAccom.} can easily be adapted to the system dynamics described in~(\ref{eq:formationFault}). The Hamiltonian dynamics can be transformed in:
\begin{equation} \label{eq:HamiltFormation}
\begin{aligned}
\begin{bmatrix}
\dot{x} \\
         \dot{\lambda} \end{bmatrix}  = \begin{bmatrix}
    L & -BB^T \\
    0 & -A^T \end{bmatrix}\begin{bmatrix}
x \\ \lambda \end{bmatrix} + \begin{bmatrix}
    H \\
    0 \end{bmatrix} + \begin{bmatrix}
    F \\
    0 \end{bmatrix} \delta
\end{aligned}.
\end{equation} 
The solution of~(\ref{eq:HamiltFormation}) at the final time $t_f$ is:
\begin{eqnarray*}
x(t_f) &=& e^{L(t_f-t_d)}x(t_d) - W(t_f,t_d) \lambda(t_d) + S(t_f,t_d)\delta + P(t_f,t_d) \\
\lambda(t_f) &=& e^{-L^T(t_f-t_d)}\lambda(t_d)
\end{eqnarray*}
where both $W(t_f,t_d)$ and $S(t_f,t_d)$ are defined as before, while:
\begin{eqnarray*}
P(t_f,t_d) &=& \int_{t_d}^{t_f} e^{L(t_f-\tau)} P d \tau.
\end{eqnarray*}
Substituting the expressions of $x(t_f)$ and $\lambda(t_f)$ in the boundary condition, and solving for $\lambda(t_d)$ leads to:
\begin{equation*}
\lambda(t_d) = R(t_f,t_d)( e^{L(t_f-t_d)}x(t_d) + H + S\delta - x_f ),
\end{equation*}
where $R(t_f,t_d)$ is defined as in~\ref{sec:optimalAccom.}. From this expression we derive the updated version of the leader input as defined in~(\ref{eq:leaderInput}).

\subsection{Robot Experiments}
\begin{figure}[h]
\begin{center}
\includegraphics[width=\columnwidth]{formation_residuals.eps}    % The printed column width is 8.4 cm.
\caption{Fault estimation filter residuals. Residuals coupled with the fault (top plot) and residuals uncoupled with the faults (bottom plot).} 
\label{fig:formation_residuals}
\end{center}
\end{figure}

\begin{figure}[h]
\begin{center}
\includegraphics[width=\columnwidth]{formation.eps}    % The printed column width is 8.4 cm.
\caption{Final formation after fault with leader accommodation (solid dots) and without final accommodation (blank circles).} 
\label{fig:formation}
\end{center}
\end{figure}



